In-Context Learning (and Unlearning) of Length Biases

Large language models have demonstrated strong capabilities to learn in-context, where exemplar input-output pairings are appended to the prompt for demonstration. However, existing work has demonstrated the ability of models to learn lexical and label biases in-context, which negatively impacts both performance and robustness of models. The impact of other statistical data biases remains under-explored, which this work aims to address. We specifically investigate the impact of length biases on in-context learning. We demonstrate that models do learn length biases in the context window for their predictions, and further empirically analyze the factors that modulate the level of bias exhibited by the model. In addition, we show that learning length information in-context can be used to counter the length bias that has been encoded in models (e.g., via fine-tuning). This reveals the power of in-context learning in debiasing model prediction behaviors without the need for costly parameter updates.

==> latex/figures/int_mrpc_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama3_8b_class2_6bins.png}
            \caption{Finetuning: $y_1$ (Blue) short demonstrations, $y_2$ (Orange) long demonstrations.}\label{fig:ft_og_mrpc}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/mrpc_16_llama3_8b_class2_6bins.png}
            \caption{Intervention: $y_1$ (Blue) long demonstrations, $y_2$ (Orange) short demonstrations.}\label{fig:int_cls_mrpc}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/mrpc_16_llama3_8b_cls2_random_6bins.png}
            \caption{Intervention: $y_1$ (Blue) and $y_2$ (Orange) demonstrations randomly sampled.}\label{fig:int_ran_mrpc}
        \end{subfigure}
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:int-hans} MRPC validation set performance on a finetuned Llama 3 (8B) model exhibiting a length bias (see \autoref{fig:ft_og_mrpc} for finetuning performance prior to intervention). \autoref{fig:int_cls_mrpc} and \autoref{fig:int_ran_mrpc} (respectively) show results on two debiasing conditions: ICL demonstrations ($k=16$) sampled from the opposite lengths from what the model saw during finetuning (i.e. $y_1$ long demonstrations, $y_2$ short demonstrations), and random sampling.}
    \end{minipage}
\end{figure*}

==> latex/figures/int_qnli_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama3_8b_class2_6bins.png}
            \caption{Finetuning: $y_1$ (Blue) short demonstrations, $y_2$ (Orange) long demonstrations.}\label{fig:ft_og_qnli}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/qnli_16_llama3_8b_class2_6bins.png}
            \caption{Intervention: $y_1$ (Blue) long demonstrations, $y_2$ (Orange) short demonstrations.}\label{fig:int_cls_qnli}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/qnli_16_llama3_8b_cls2_random_6bins.png}
            \caption{Intervention: $y_1$ (Blue) and $y_2$ (Orange) demonstrations randomly sampled.}\label{fig:int_ran_qnli}
        \end{subfigure}
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:int-hans} QNLI validation set performance on a finetuned Llama 3 (8B) model exhibiting a length bias (see \autoref{fig:ft_og_qnli} for finetuning performance prior to intervention). \autoref{fig:int_cls_qnli} and \autoref{fig:int_ran_qnli} (respectively) show results on two debiasing conditions: ICL demonstrations ($k=16$) sampled from the opposite lengths from what the model saw during finetuning (i.e. $y_1$ long demonstrations, $y_2$ short demonstrations), and random sampling.}
    \end{minipage}
\end{figure*}

==> latex/figures/int_rte_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama3_8b_class2_6bins.png}
            \caption{Finetuning: $y_1$ (Blue) short demonstrations, $y_2$ (Orange) long demonstrations.}\label{fig:ft_og_rte}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/rte_16_llama3_8b_class2_6bins.png}
            \caption{Intervention: $y_1$ (Blue) long demonstrations, $y_2$ (Orange) short demonstrations.}\label{fig:int_cls_rte}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/rte_16_llama3_8b_cls2_random_6bins.png}
            \caption{Intervention: $y_1$ (Blue) and $y_2$ (Orange) demonstrations randomly sampled.}\label{fig:int_ran_rte}
        \end{subfigure}
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:int-rte} RTE validation set performance on a finetuned Llama 3 (8B) model exhibiting a length bias (see \autoref{fig:ft_og_rte} for finetuning performance prior to intervention). \autoref{fig:int_cls_rte} and \autoref{fig:int_ran_rte} (respectively) show results on two debiasing conditions: ICL demonstrations ($k=16$) sampled from the opposite lengths from what the model saw during finetuning (i.e. $y_1$ long demonstrations, $y_2$ short demonstrations), and random sampling.}
    \end{minipage}
\end{figure*}

==> latex/figures/int_sst2_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama3_8b_class2_6bins.png}
            \caption{Finetuning: $y_1$ (Blue) short demonstrations, $y_2$ (Orange) long demonstrations.}\label{fig:ft_og_sst2}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/sst2_16_llama3_8b_class2_6bins.png}
            \caption{Intervention: $y_1$ (Blue) long demonstrations, $y_2$ (Orange) short demonstrations.}\label{fig:int_cls_sst2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.31\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/int/sst2_16_llama3_8b_cls2_random_6bins.png}
            \caption{Intervention: $y_1$ (Blue) and $y_2$ (Orange) demonstrations randomly sampled.}\label{fig:int_ran_sst2}
        \end{subfigure}
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:int-hans} SST2 validation set performance on a finetuned Llama 3 (8B) model exhibiting a length bias (see \autoref{fig:ft_og_sst2} for finetuning performance prior to intervention). \autoref{fig:int_cls_sst2} and \autoref{fig:int_ran_sst2} (respectively) show results on two debiasing conditions: ICL demonstrations ($k=16$) sampled from the opposite lengths from what the model saw during finetuning (i.e. $y_1$ long demonstrations, $y_2$ short demonstrations), and random sampling.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_hans_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/hans_16_gpt_2dot7b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/hans_16_gpt_2dot7b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/hans_16_gpt_2dot7b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/hans_16_gpt_2dot7b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the Hans dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_hans_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/hans_16_gpt_2dot7b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/hans_16_gpt_2dot7b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/hans_16_gpt_2dot7b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/hans_16_gpt_2dot7b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the Hans dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_mrpc_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/mrpc_16_gpt_2dot7b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/mrpc_16_gpt_2dot7b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/mrpc_16_gpt_2dot7b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/mrpc_16_gpt_2dot7b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the mrpc dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_mrpc_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/mrpc_16_gpt_2dot7b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/mrpc_16_gpt_2dot7b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/mrpc_16_gpt_2dot7b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/mrpc_16_gpt_2dot7b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the mrpc dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_paws_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/en_16_gpt_2dot7b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/en_16_gpt_2dot7b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/en_16_gpt_2dot7b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/en_16_gpt_2dot7b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the PAWS dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_paws_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/en_16_gpt_2dot7b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/en_16_gpt_2dot7b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/en_16_gpt_2dot7b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/en_16_gpt_2dot7b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the PAWS dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_qnli_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/qnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/qnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/qnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/qnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the qnli dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_qnli_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/qnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/qnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/qnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/qnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the qnli dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_rte_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/rte_16_gpt_2dot7b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/rte_16_gpt_2dot7b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/rte_16_gpt_2dot7b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/rte_16_gpt_2dot7b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the rte dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_rte_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/rte_16_gpt_2dot7b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/rte_16_gpt_2dot7b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/rte_16_gpt_2dot7b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/rte_16_gpt_2dot7b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the rte dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_sst2_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/sst2_16_gpt_2dot7b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/sst2_16_gpt_2dot7b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/sst2_16_gpt_2dot7b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/sst2_16_gpt_2dot7b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the sst2 dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_sst2_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/sst2_16_gpt_2dot7b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/sst2_16_gpt_2dot7b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/sst2_16_gpt_2dot7b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/sst2_16_gpt_2dot7b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the sst2 dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_wnli_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/wnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/wnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/wnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/wnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the wnli dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/gpt_wnli_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/wnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/wnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/wnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/wnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:gpt-len-qnli}GPT performance across different length sampling on the wnli dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_hans_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/hans_16_llama3_8b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/hans_16_llama3_8b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/hans_16_llama3_8b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/hans_16_llama3_8b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the Hans dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_hans_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/hans_16_llama3_8b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/hans_16_llama3_8b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/hans_16_llama3_8b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/hans_16_llama3_8b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the Hans dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_mrpc_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/mrpc_16_llama3_8b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/mrpc_16_llama3_8b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/mrpc_16_llama3_8b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/mrpc_16_llama3_8b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the mprc dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_mrpc_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/mrpc_16_llama3_8b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/mrpc_16_llama3_8b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/mrpc_16_llama3_8b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/mrpc_16_llama3_8b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the mrpc dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_paws_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/en_16_llama3_8b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/en_16_llama3_8b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/en_16_llama3_8b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/en_16_llama3_8b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the PAWS dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_paws_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/en_16_llama3_8b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/en_16_llama3_8b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/en_16_llama3_8b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/en_16_llama3_8b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the PAWS dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_qnli_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/qnli_16_llama3_8b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/qnli_16_llama3_8b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/qnli_16_llama3_8b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/qnli_16_llama3_8b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the qnli dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_qnli_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/qnli_16_llama3_8b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/qnli_16_llama3_8b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/qnli_16_llama3_8b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/qnli_16_llama3_8b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the qnli dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_rte_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/rte_16_llama3_8b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/rte_16_llama3_8b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/rte_16_llama3_8b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/rte_16_llama3_8b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the rte dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_rte_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/rte_16_llama3_8b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/rte_16_llama3_8b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/rte_16_llama3_8b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/rte_16_llama3_8b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the rte dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_sst2_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/sst2_16_llama3_8b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/sst2_16_llama3_8b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/sst2_16_llama3_8b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/sst2_16_llama3_8b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the sst2 dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_sst2_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/sst2_16_llama3_8b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/sst2_16_llama3_8b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/sst2_16_llama3_8b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/sst2_16_llama3_8b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the sst2 dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_wnli_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/wnli_16_llama3_8b_class1_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/wnli_16_llama3_8b_class1_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/wnli_16_llama3_8b_class1_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/wnli_16_llama3_8b_class1_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the wnli dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/len_diff_tex/llama3_wnli_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/tail/wnli_16_llama3_8b_class2_6bins.png}
            \caption{tail}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/25/wnli_16_llama3_8b_class2_6bins.png}
            \caption{$25\%$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/50/wnli_16_llama3_8b_class2_6bins.png}
            \caption{$50\%$}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/len_diff/75/wnli_16_llama3_8b_class2_6bins.png}
            \caption{$75\%$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:llama3-len-qnli}Llama3 performance across different length sampling on the wnli dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/lineplots/ex_app.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_llama3_8b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_llama3_8b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_llama3_8b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_llama3_8b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of Llama3 (8B) across different numbers of demonstrations on the Hans dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_llama3_8b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_llama3_8b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_llama3_8b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_llama3_8b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of Llama3 (8B) across different numbers of demonstrations on the RTE dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_llama3_8b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_llama3_8b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_llama3_8b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_llama3_8b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of Llama3 (8B) across different numbers of demonstrations on the WNLI dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
                \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_llama3_8b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_llama3_8b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_llama3_8b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_llama3_8b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of Llama3 (8B) across different numbers of demonstrations on the QNLI dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_llama3_8b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_llama3_8b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_llama3_8b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_llama3_8b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of Llama3 (8B) across different numbers of demonstrations on the MPRC dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_llama3_8b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_llama3_8b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_llama3_8b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_llama3_8b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of Llama3 (8B) across different numbers of demonstrations on the SST2 dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

==> latex/figures/lineplots/ex_app_gpt.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_gpt_2dot7b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_gpt_2dot7b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_gpt_2dot7b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/hans_gpt_2dot7b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of GPT-Neo (2.7B) across different numbers of demonstrations on the Hans dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_gpt_2dot7b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_gpt_2dot7b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_gpt_2dot7b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/rte_gpt_2dot7b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of GPT-Neo (2.7B) across different numbers of demonstrations on the RTE dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_gpt_2dot7b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_gpt_2dot7b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_gpt_2dot7b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/wnli_gpt_2dot7b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of GPT-Neo (2.7B) across different numbers of demonstrations on the WNLI dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
                \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_gpt_2dot7b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_gpt_2dot7b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_gpt_2dot7b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/qnli_gpt_2dot7b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of GPT-Neo (2.7B) across different numbers of demonstrations on the QNLI dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_gpt_2dot7b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_gpt_2dot7b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_gpt_2dot7b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/mrpc_gpt_2dot7b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of GPT-Neo (2.7B) across different numbers of demonstrations on the MPRC dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_gpt_2dot7b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_gpt_2dot7b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_gpt_2dot7b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/sst2_gpt_2dot7b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of GPT-Neo (2.7B) across different numbers of demonstrations on the SST2 dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}


\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/en_gpt_2dot7b_class2_cls1.png}
            \caption{$y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/en_gpt_2dot7b_random_cls1.png}
            \caption{$y_1$ (random sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/en_gpt_2dot7b_class2_cls2.png}
            \caption{$y_2$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/examples/en_gpt_2dot7b_random_cls1.png}
            \caption{$y_2$ (random sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_ex} Validation performance of GPT-Neo (2.7B) across different numbers of demonstrations on the PAWS dataset. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class. The conditions that introduce length bias in the context window (a and c subfigures) demonstrate a larger spread between performance on short and long validation instances, indicating greater potential to learn bias with longer contexts.}
    \end{minipage}
\end{figure}

==> latex/figures/lineplots/length_app.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/rte_llama3_8b_class2_cls1.png}
            \caption{RTE: \\ $y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/rte_llama3_8b_class2_cls2.png}
            \caption{RTE: \\ $y_2$ (biased sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/mrpc_llama3_8b_class2_cls1.png}
            \caption{MRPC: \\ $y_1$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/mrpc_llama3_8b_class2_cls2.png}
            \caption{MRPC: \\ $y_2$ (biased sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:len} Validation performance across different data sampling percentages using Llama 3 (8B). In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class, with Bin 0 containing the shortest demonstrations and Bin 5 containing the longest demonstrations.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/rte_gpt_2dot7b_class2_cls1.png}
            \caption{RTE: \\ $y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/rte_gpt_2dot7b_class2_cls2.png}
            \caption{RTE: \\ $y_2$ (biased sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/mrpc_gpt_2dot7b_class2_cls1.png}
            \caption{MRPC: \\ $y_1$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/length/mrpc_gpt_2dot7b_class2_cls2.png}
            \caption{MRPC: \\ $y_2$ (biased sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:len} Validation performance across different data sampling percentages using GPT-Neo 2.7B. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class, with Bin 0 containing the shortest demonstrations and Bin 5 containing the longest demonstrations. }
    \end{minipage}
\end{figure}

==> latex/figures/lineplots/param_app_old.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/en_opt_class2_cls1.png}
            \caption{PAWS-X$_{EN}$: \\ $y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/en_opt_class2_cls2.png}
            \caption{PAWS-X$_{EN}$: \\ $y_2$ (biased sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/hans_opt_class2_cls1.png}
            \caption{Hans: \\ $y_1$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/hans_opt_class2_cls2.png}
            \caption{Hans: \\ $y_2$ (biased sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_params} Validation performance across different numbers of model parameters using the OPT model family. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class, with Bin 0 containing the shortest demonstrations and Bin 5 containing the longest demonstrations. Additional results can be found in the Appendix.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/rte_opt_class2_cls1.png}
            \caption{RTE: \\ $y_1$ (short instances)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/rte_opt_class2_cls2.png}
            \caption{RTE: \\ $y_2$ (long)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/wnli_opt_class2_cls1.png}
            \caption{WNLI: \\ $y_1$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/wnli_opt_class2_cls2.png}
            \caption{WNLI: \\ $y_2$ (biased sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_params} Validation performance across different numbers of model parameters using the OPT model family. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class, with Bin 0 containing the shortest demonstrations and Bin 5 containing the longest demonstrations. Additional results can be found in the Appendix.}
    \end{minipage}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/qnli_opt_class2_cls1.png}
            \caption{QNLI: \\ $y_1$ (biased sampling)}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/qnli_opt_class2_cls2.png}
            \caption{QNLI: \\ $y_2$ (biased sampling)}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/mrpc_opt_class2_cls1.png}
            \caption{MRPC: \\ $y_1$ (biased sampling)}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/parameters/mrpc_opt_class2_cls2.png}
            \caption{MRPC: \\ $y_2$ (biased sampling)}\label{fig:image4}
        \end{subfigure}%
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \centering
        \vspace{2mm}
            \begin{subfigure}{0.7 \linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/lineplots/legend.pdf}
        \end{subfigure}%
    \end{minipage}
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:num_params} Validation performance across different numbers of model parameters using the OPT model family. In this figure, in-context examples from $y_2$ were sampled from long instances, and in-context examples from $y_1$ were sampled from short instances. Each subfigure shows results on the validation instances in the respective class, with Bin 0 containing the shortest demonstrations and Bin 5 containing the longest demonstrations. Additional results can be found in the Appendix.}
    \end{minipage}
\end{figure}

==> latex/figures/num_ex_tex/gpt_hans_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_2_gpt_2dot7b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_4_gpt_2dot7b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_8_gpt_2dot7b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_16_gpt_2dot7b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_24_gpt_2dot7b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_32_gpt_2dot7b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance across different parameter values on the hans dataset under the class1 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_hans_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_2_gpt_2dot7b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_4_gpt_2dot7b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_8_gpt_2dot7b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_16_gpt_2dot7b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_24_gpt_2dot7b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_32_gpt_2dot7b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance on gpt-neo-2.7b on the hans dataset under the class2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_hans_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_2_gpt_2dot7b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_4_gpt_2dot7b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_8_gpt_2dot7b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_16_gpt_2dot7b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_24_gpt_2dot7b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_32_gpt_2dot7b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance across different parameter values on the hans dataset under the random long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_mrpc_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_2_gpt_2dot7b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_4_gpt_2dot7b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_8_gpt_2dot7b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_16_gpt_2dot7b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_24_gpt_2dot7b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_32_gpt_2dot7b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different parameter values on the mrpc dataset under the class1 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_mrpc_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_2_gpt_2dot7b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_4_gpt_2dot7b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_8_gpt_2dot7b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_16_gpt_2dot7b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_24_gpt_2dot7b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_32_gpt_2dot7b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different parameter values on the mrpc dataset under the class2 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_mrpc_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_2_gpt_2dot7b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_4_gpt_2dot7b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_8_gpt_2dot7b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_16_gpt_2dot7b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_24_gpt_2dot7b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_32_gpt_2dot7b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different parameter values on the mrpc dataset under the random long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_paws_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_2_gpt_2dot7b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_4_gpt_2dot7b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_8_gpt_2dot7b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_16_gpt_2dot7b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_24_gpt_2dot7b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_32_gpt_2dot7b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance across different parameter values on the PAWS dataset under the class1 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_paws_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_2_gpt_2dot7b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_4_gpt_2dot7b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_8_gpt_2dot7b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_16_gpt_2dot7b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_24_gpt_2dot7b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_32_gpt_2dot7b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance on gpt-neo-2.7b on the PAWS dataset under the class2 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_paws_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_2_gpt_2dot7b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_4_gpt_2dot7b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_8_gpt_2dot7b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_16_gpt_2dot7b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_24_gpt_2dot7b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_32_gpt_2dot7b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance across different parameter values on the PAWS dataset under the random long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_qnli_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_2_gpt_2dot7b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_4_gpt_2dot7b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_8_gpt_2dot7b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_24_gpt_2dot7b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_32_gpt_2dot7b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different parameter values on the qnli dataset under the class1 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_qnli_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_2_gpt_2dot7b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_4_gpt_2dot7b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_8_gpt_2dot7b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_24_gpt_2dot7b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_32_gpt_2dot7b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different parameter values on the qnli dataset under the class2 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_qnli_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_2_gpt_2dot7b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_4_gpt_2dot7b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_8_gpt_2dot7b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_16_gpt_2dot7b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_24_gpt_2dot7b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_32_gpt_2dot7b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different parameter values on the qnli dataset under the random long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_rte_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_2_gpt_2dot7b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_4_gpt_2dot7b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_8_gpt_2dot7b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_16_gpt_2dot7b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_24_gpt_2dot7b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_32_gpt_2dot7b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different parameter values on the rte dataset under the class1 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_rte_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_2_gpt_2dot7b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_4_gpt_2dot7b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_8_gpt_2dot7b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_16_gpt_2dot7b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_24_gpt_2dot7b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_32_gpt_2dot7b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different parameter values on the rte dataset under the class2 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_rte_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_2_gpt_2dot7b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_4_gpt_2dot7b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_8_gpt_2dot7b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_16_gpt_2dot7b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_24_gpt_2dot7b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_32_gpt_2dot7b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different parameter values on the rte dataset under the random long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_sst2_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_2_gpt_2dot7b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_4_gpt_2dot7b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_8_gpt_2dot7b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_16_gpt_2dot7b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_24_gpt_2dot7b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_32_gpt_2dot7b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different parameter values on the sst2 dataset under the class1 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_sst2_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_2_gpt_2dot7b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_4_gpt_2dot7b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_8_gpt_2dot7b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_16_gpt_2dot7b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_24_gpt_2dot7b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_32_gpt_2dot7b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different parameter values on the sst2 dataset under the class2 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_sst2_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_2_gpt_2dot7b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_4_gpt_2dot7b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_8_gpt_2dot7b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_16_gpt_2dot7b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_24_gpt_2dot7b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_32_gpt_2dot7b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different parameter values on the sst2 dataset under the random long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_wnli_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_2_gpt_2dot7b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_4_gpt_2dot7b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_8_gpt_2dot7b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_16_gpt_2dot7b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_24_gpt_2dot7b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_32_gpt_2dot7b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different parameter values on the wnli dataset under the class1 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_wnli_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_2_gpt_2dot7b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_4_gpt_2dot7b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_8_gpt_2dot7b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_16_gpt_2dot7b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_24_gpt_2dot7b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_32_gpt_2dot7b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different parameter values on the wnli dataset under the class2 long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/gpt_wnli_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_2_gpt_2dot7b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_4_gpt_2dot7b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_8_gpt_2dot7b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_16_gpt_2dot7b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_24_gpt_2dot7b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_32_gpt_2dot7b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different parameter values on the wnli dataset under the random long condition using gpt neo 2.7b.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_hans_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_2_llama3_8b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_4_llama3_8b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_8_llama3_8b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_16_llama3_8b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_24_llama3_8b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_32_llama3_8b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance across different parameter values on the Hans dataset under the class1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_hans_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_2_llama3_8b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_4_llama3_8b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_8_llama3_8b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_16_llama3_8b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_24_llama3_8b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_32_llama3_8b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance on Llama3 on the Hans dataset under the class2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_hans_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_2_llama3_8b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_4_llama3_8b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_8_llama3_8b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_16_llama3_8b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_24_llama3_8b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/hans_32_llama3_8b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance across different parameter values on the Hans dataset under the random long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_mrpc_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_2_llama3_8b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_4_llama3_8b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_8_llama3_8b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_16_llama3_8b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_24_llama3_8b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_32_llama3_8b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different parameter values on the mrpc dataset under the class1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_mrpc_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_2_llama3_8b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_4_llama3_8b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_8_llama3_8b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_16_llama3_8b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_24_llama3_8b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_32_llama3_8b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different parameter values on the mrpc dataset under the class2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_mrpc_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_2_llama3_8b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_4_llama3_8b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_8_llama3_8b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_16_llama3_8b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_24_llama3_8b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/mrpc_32_llama3_8b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different parameter values on the mrpc dataset under the random long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_paws_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_2_llama3_8b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_4_llama3_8b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_8_llama3_8b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_16_llama3_8b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_24_llama3_8b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_32_llama3_8b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance across different parameter values on the PAWS dataset under the class1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_paws_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_2_llama3_8b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_4_llama3_8b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_8_llama3_8b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_16_llama3_8b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_24_llama3_8b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_32_llama3_8b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance on llama3 on the PAWS dataset under the class2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_paws_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_2_llama3_8b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_4_llama3_8b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_8_llama3_8b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/en_16_llama3_8b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_24_llama3_8b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/en_32_llama3_8b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance across different parameter values on the PAWS dataset under the random condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_qnli_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_2_llama3_8b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_4_llama3_8b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_8_llama3_8b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_16_llama3_8b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_24_llama3_8b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_32_llama3_8b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different parameter values on the qnli dataset under the class1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_qnli_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_2_llama3_8b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_4_llama3_8b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_8_llama3_8b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_16_llama3_8b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_24_llama3_8b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_32_llama3_8b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different parameter values on the qnli dataset under the class2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_qnli_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_2_llama3_8b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_4_llama3_8b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_8_llama3_8b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_16_llama3_8b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_24_llama3_8b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/qnli_32_llama3_8b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different parameter values on the qnli dataset under the random long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_rte_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_2_llama3_8b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_4_llama3_8b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_8_llama3_8b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_16_llama3_8b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_24_llama3_8b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_32_llama3_8b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different parameter values on the rte dataset under the class1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_rte_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_2_llama3_8b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_4_llama3_8b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_8_llama3_8b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_16_llama3_8b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_24_llama3_8b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_32_llama3_8b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different parameter values on the rte dataset under the class2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_rte_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_2_llama3_8b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_4_llama3_8b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_8_llama3_8b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_16_llama3_8b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_24_llama3_8b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/rte_32_llama3_8b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different parameter values on the rte dataset under the random long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_sst2_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_2_llama3_8b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_4_llama3_8b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_8_llama3_8b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_16_llama3_8b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_24_llama3_8b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_32_llama3_8b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different parameter values on the sst2 dataset under the class1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_sst2_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_2_llama3_8b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_4_llama3_8b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_8_llama3_8b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_16_llama3_8b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_24_llama3_8b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_32_llama3_8b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different parameter values on the sst2 dataset under the class2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_sst2_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_2_llama3_8b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_4_llama3_8b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_8_llama3_8b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_16_llama3_8b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_24_llama3_8b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/sst2_32_llama3_8b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different parameter values on the sst2 dataset under the random long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_wnli_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_2_llama3_8b_class1_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_4_llama3_8b_class1_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_8_llama3_8b_class1_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_16_llama3_8b_class1_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_24_llama3_8b_class1_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_32_llama3_8b_class1_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different parameter values on the wnli dataset under the class1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_wnli_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_2_llama3_8b_class2_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_4_llama3_8b_class2_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_8_llama3_8b_class2_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_16_llama3_8b_class2_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_24_llama3_8b_class2_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_32_llama3_8b_class2_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different parameter values on the wnli dataset under the class2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/num_ex_tex/llama3_wnli_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_2_llama3_8b_random_6bins.png}
            \caption{$k=2$}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_4_llama3_8b_random_6bins.png}
            \caption{$k=4$}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_8_llama3_8b_random_6bins.png}
            \caption{$k=8$}\label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.16\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_16_llama3_8b_random_6bins.png}
            \caption{$k=16$}\label{fig:image4}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_24_llama3_8b_random_6bins.png}
        \caption{$k=24$}\label{fig:image4}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.16\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/num_ex/wnli_32_llama3_8b_random_6bins.png}
        \caption{$k=32$}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different parameter values on the wnli dataset under the random long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_hans_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_350m_class1_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_1dot3b_class1_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_2dot7b_class1_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-hans}Performance across different parameter values on the Hans dataset under the class 1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_hans_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_350m_class2_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_1dot3b_class2_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_2dot7b_class2_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-hans-cls2}Performance across different parameter values on the Hans dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_hans_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_350m_random_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_1dot3b_random_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_2dot7b_random_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/hans_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-hans}Performance across different parameter values on the Hans dataset under the random condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_mrpc_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_350m_class1_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_1dot3b_class1_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_2dot7b_class1_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-mrpc}Performance across different parameter values on the MRPC dataset under the class 1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_mrpc_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_350m_class2_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_1dot3b_class2_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_2dot7b_class2_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-mrpc}Performance across different parameter values on the MRPC dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_mrpc_rand.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_350m_random_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_1dot3b_random_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_2dot7b_random_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/mrpc_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-mrpc}Performance across different parameter values on the MRPC dataset under the random condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_paws_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_350m_class1_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_1dot3b_class1_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_2dot7b_class1_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-paws}Performance across different parameter values on the PAWS-X$_{\textsc{EN}}$ dataset under class 1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_paws_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_350m_class2_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_1dot3b_class2_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_2dot7b_class2_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-paws-cls2}Performance across different parameter values on the PAWS-X$_{\textsc{EN}}$ dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_paws_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_350m_random_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_1dot3b_random_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_2dot7b_random_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/en_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-paws}Performance across different parameter values on the PAWS-X$_{\textsc{EN}}$ dataset under the random condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_qnli_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_350m_class1_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_1dot3b_class1_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_2dot7b_class1_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-qnli}Performance across different parameter values on the QNLI dataset under the class 1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_qnli_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_350m_class2_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_1dot3b_class2_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_2dot7b_class2_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-qnli}Performance across different parameter values on the QNLI dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_qnli_rand.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_350m_random_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_1dot3b_random_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_2dot7b_random_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/qnli_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-qnli}Performance across different parameter values on the QNLI dataset under the random condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_rte_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_350m_class1_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_1dot3b_class1_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_2dot7b_class1_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-rte}Performance across different parameter values on the RTE dataset under the class 1 condition.}
    \end{minipage}
\end{figure*}


==> latex/figures/opt_rte_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_350m_class2_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_1dot3b_class2_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_2dot7b_class2_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-rte}Performance across different parameter values on the RTE dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}


==> latex/figures/opt_rte_rand.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_350m_random_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_1dot3b_random_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_2dot7b_random_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/rte_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-rte}Performance across different parameter values on the RTE dataset under the random conddition.}
    \end{minipage}
\end{figure*}


==> latex/figures/opt_sst2_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_350m_class1_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_1dot3b_class1_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_2dot7b_class1_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-sst2}Performance across different parameter values on the SST2 dataset under the class 1 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_sst2_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_350m_class2_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_1dot3b_class2_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_2dot7b_class2_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-sst2}Performance across different parameter values on the SST2 dataset under the class 2 condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_sst2_rand.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_350m_random_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_1dot3b_random_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_2dot7b_random_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/sst2_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-sst2}Performance across different parameter values on the SST2 dataset under the random condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_wnli_cls1.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_350m_class1_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_1dot3b_class1_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_2dot7b_class1_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-wnli}Performance across different parameter values on the WNLI dataset under the class 1 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_wnli_cls2.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_350m_class2_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_1dot3b_class2_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_2dot7b_class2_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-wnli}Performance across different parameter values on the WNLI dataset under the class 2 long condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/opt_wnli_rand.tex <==
\begin{figure*}
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_350m_random_6bins.png}
            \caption{OPT 350M}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_1dot3b_random_6bins.png}
            \caption{OPT 1.3B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_2dot7b_random_6bins.png}
            \caption{OPT 2.7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.245\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/cumulative_acc/wnli_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:opt-wnli}Performance across different parameter values on the WNLI dataset under the random condition.}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_ft_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the Hans dataset. For each graph, $y_1$ (Blue) was sampled from the short instances, and $y_2$ (Orange) was sampled from the long instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the RTE dataset. For each graph, $y_1$ (Blue) was sampled from the short instances, and $y_2$ (Orange) was sampled from the long instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the QNLI dataset. For each graph, $y_1$ (Blue) was sampled from the short instances, and $y_2$ (Orange) was sampled from the long instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the WNLI dataset. For each graph, $y_1$ (Blue) was sampled from the short instances, and $y_2$ (Orange) was sampled from the long instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the MPRC dataset. For each graph, $y_1$ (Blue) was sampled from the short instances, and $y_2$ (Orange) was sampled from the long instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the PAWS dataset. For each graph, $y_1$ (Blue) was sampled from the short instances, and $y_2$ (Orange) was sampled from the long instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the SST2 dataset. For each graph, $y_1$ (Blue) was sampled from the short instances, and $y_2$ (Orange) was sampled from the long instances.}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_ft_clsl1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the Hans dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the RTE dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the QNLI dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the WNLI dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the MPRC dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the PAWS dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the SST2 dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_ft_hans_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the Hans dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the RTE dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/qnl_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the QNLI dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the WNLI dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the MPRC dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the PAWS dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the SST2 dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_ft_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/hans_200_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the Hans dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/rte_200_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft-hans}Finetuning validation performance across different models on the RTE dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/qnli_200_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/qnl_200_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the QNLI dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/wnli_200_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the WNLI dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/mrpc_200_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the MPRC dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/paws_200_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the PAWS dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/ft/sst2_200_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-ft}Finetuning validation performance across different models on the SST2 dataset. For each graph, $y_1$ (Blue) was sampled from the long instances, and $y_2$ (Orange) was sampled from the short instances.}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_hans_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance across different models on the Hans dataset ($y_1$ long demonstrations, $y_2$ short demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_hans_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/hans_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-hans}Performance across different models on the Hans dataset ($y_1$ randomly sampled demonstrations, $y_2$ randomly sampled demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_mrpc_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different models on the MRPC dataset ($y_1$ long demonstrations, $y_2$ short demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_mrpc_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_llama3_8b_class2_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_llama2_7b_class2_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_mistral_7b_class2_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_gpt_2dot7b_class2_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different models on the MRPC dataset ($y_1$ short demonstrations, $y_2$ long demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_mrpc_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/mrpc_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-mrpc}Performance across different models on the Hans dataset ($y_1$ randomly sampled demonstrations, $y_2$ randomly sampled demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_paws_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance across different models on the PAWS-X$_{\textsc{EN}}$ dataset ($y_1$ long demonstrations, $y_2$ short demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_paws_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/en_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-en}Performance across different models on the PAWS-X$_{\textsc{EN}}$ dataset ($y_1$ randomly sampled demonstrations, $y_2$ randomly sampled demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_qnli_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different models on the QNLI dataset ($y_1$ long demonstrations, $y_2$ short demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_qnli_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_llama3_8b_class2_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_llama2_7b_class2_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_mistral_7b_class2_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_gpt_2dot7b_class2_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different models on the QNLI dataset ($y_1$ short demonstrations, $y_2$ long demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_qnli_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/qnli_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-qnli}Performance across different models on the Hans dataset ($y_1$ randomly sampled demonstrations, $y_2$ randomly sampled demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_rte_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different models on the RTE dataset ($y_1$ long demonstrations, $y_2$ short demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_rte_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_llama3_8b_class2_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_llama2_7b_class2_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_mistral_7b_class2_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_gpt_2dot7b_class2_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different models on the Hans dataset ($y_1$ short demonstrations, $y_2$ long demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_rte_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/rte_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-rte}Performance across different models on the Hans dataset ($y_1$ randomly sampled demonstrations, $y_2$ randomly sampled demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_sst2_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different models on the SST2 dataset ($y_1$ long demonstrations, $y_2$ short demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_sst2_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_llama3_8b_class2_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_llama2_7b_class2_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_mistral_7b_class2_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_gpt_2dot7b_class2_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different models on the SST2 dataset ($y_1$ short demonstrations, $y_2$ long demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_sst2_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/sst2_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-sst2}Performance across different models on the SST2 dataset ($y_1$ randomly sampled demonstrations, $y_2$ randomly sampled demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_wnli_cls1.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_llama3_8b_class1_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_llama2_7b_class1_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_mistral_7b_class1_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_opt_6dot7b_class1_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_gpt_2dot7b_class1_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different models on the WNLI dataset ($y_1$ long demonstrations, $y_2$ short demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_wnli_cls2.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_llama3_8b_class2_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_llama2_7b_class2_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_mistral_7b_class2_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_opt_6dot7b_class2_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_gpt_2dot7b_class2_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different models on the WNLI dataset ($y_1$ short demonstrations, $y_2$ long demonstrations).}
    \end{minipage}
\end{figure*}

==> latex/figures/q1_icl_wnli_rand.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{\linewidth}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_llama3_8b_random_6bins.png}
            \caption{Llama3 8B}\label{fig:image1}
        \end{subfigure}% 
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_llama2_7b_random_6bins.png}
            \caption{Llama2 7B}\label{fig:image2}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_mistral_7b_random_6bins.png}
            \caption{Mistral 7B}\label{fig:image3}
        \end{subfigure}
        \begin{subfigure}{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_opt_6dot7b_random_6bins.png}
            \caption{OPT 6.7B}\label{fig:image4}
        \end{subfigure}% 
        \begin{subfigure}{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{latex/figures/q1_icl/wnli_gpt_2dot7b_random_6bins.png}
        \caption{GPT Neo 2.7B}\label{fig:image4}
        \end{subfigure}% 
    \end{minipage}% 
    \hfill
    \begin{minipage}[c]{\linewidth}
        \caption{\label{fig:q1-icl-wnli}Performance across different models on the WNLI dataset ($y_1$ randomly sampled demonstrations, $y_2$ randomly sampled demonstrations).}
    \end{minipage}
\end{figure*}
